Shape-driven Coordinate Ordering for Star Glyph Sets via Reinforcement Learning

We present a neural optimization model trained with reinforcement learning to solve the coordinate ordering problem for sets of star glyphs. Given a set of star glyphs associated to multiple class labels, we propose to use shape context descriptors to measure the perceptual distance between pairs of glyphs, and use the derived silhouette coefficient to measure the perception of class separability within the entire set. To find the optimal coordinate order for the given set, we train a neural network using reinforcement learning to reward orderings with high silhouette coefficients. The network consists of an encoder and a decoder with an attention mechanism. The encoder employs a recurrent neural network (RNN) to encode input shape and class information, while the decoder together with the attention mechanism employs another RNN to output a sequence with the new coordinate order. In addition, we introduce a neural network to efficiently estimate the similarity between shape context descriptors, which allows to speed up the computation of silhouette coefficients and thus the training of the axis ordering network. Two user studies demonstrate that the orders provided by our method are preferred by users for perceiving class separation. We tested our model on different settings to show its robustness and generalization abilities and demonstrate that it allows to order input sets with unseen data size, data dimension, or number of classes. We also demonstrate that our model can be adapted to coordinate ordering of other types of plots such as RadViz by replacing the proposed shape-aware silhouette coefficient with the corresponding quality metric to guide network training.

==> figures/RNN_table.tex <==
\begin{table}[H]%
	\caption{Decoder RNN module structure.}
	\label{tab:rnn}
	\begin{minipage}{\columnwidth}
		\begin{center}
		\noindent\begin{tabular}{c}
			Actor
		\end{tabular}
		
		\noindent\begin{tabular}{l|l|l}
			\hline
			Layer & Input dim & Output dim  \\
            \hline
			GRU & $2$ & $256$ \\ 
            \hline
            \hline
			Layer & \multicolumn{1}{l}{Probability} \\
            \hline
			GRU hidden dropout & \multicolumn{1}{l}{$0.1$} \\
            \hline
			GRU output dropout & \multicolumn{1}{l}{$0.1$} \\
			\hline
		\end{tabular}

		\noindent\begin{tabular}{c}
			Critic
		\end{tabular}

		\noindent\begin{tabular}{l|l|l}
			\hline
			Layer & Input dim & Output dim  \\
            \hline
			GRU & $2$ & $256$ \\
            \hline
		\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%

==> figures/actor_attn_table.tex <==
\begin{table}[H]%
	\caption{Actor attention module structure. }%\ok{What about the layers?}}
	\label{tab:actor}
	\begin{minipage}{\columnwidth}
		\begin{center}
        \begin{tabular}{l|l}
			\hline
			Parameter & Size  \\
			\hline
			$v_a$ & $1\times 256$ \\
			\hline
			$v_c$ & $1\times 256$ \\
			\hline
			$W_a$ & $256\times 512$ \\
			\hline
            $W_c$ & $256\times 512$ \\
			\hline
		\end{tabular}
		\end{center}
	\end{minipage}
\end{table}%


==> figures/critic_attn_table.tex <==
\begin{table}[H]%
	\caption{Critic glimpse module structure.}
	\label{tab:critic}
	\begin{minipage}{\columnwidth}
		\begin{center}
		\noindent\begin{tabular}{l|l|l}
			\hline
			Parameter & \multicolumn{1}{l}{Size} \\
			\hline
			$v_g$ & \multicolumn{1}{l}{ $1\times 256$} \\
			\hline
			$W_g$ & \multicolumn{1}{l}{ $256\times 512$} \\
			\hline
			\hline
			Layer & Input dim & Output dim  \\
			\hline
			Linear & 256 & 256 \\
			\hline
			ReLU & \multicolumn{1}{l}{-} \\
			\hline
			Linear & 256 & 1 \\
			\hline
		\end{tabular}
		
		\end{center}
	\end{minipage}
\end{table}%

==> figures/embed_table.tex <==
\begin{table}[H]%
    \caption{Embedded RNN module structure.}
    \label{tab:embed}
    \begin{minipage}{\columnwidth}
        \begin{center}        
        \noindent\begin{tabular}{l|l|l}
            \hline
            Layer & Input dim & Output dim  \\
            \hline
            GRU & $2$ & $256$ \\ 
            \hline
            \hline
            Layer & \multicolumn{1}{l}{Probability} \\
            \hline
            GRU hidden dropout & \multicolumn{1}{l}{$0.1$} \\
            \hline
        \end{tabular}

        \end{center}
    \end{minipage}
\end{table}%

==> figures/label_comp.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width=0.95\linewidth]{images/l_curve.pdf}
	\caption{Comparison between different representations of cluster information.}
	\label{fig:label_comp}
\end{figure}


==> figures/network_structure.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.45\textwidth]{images/network_structure.pdf}
\caption{Network structure of (a) the actor network and (b) the critic network. $n$ is the number of coordinates, and $\Rightarrow$ represents an empty initial input of the RNN module.}
\label{fig:network_structure}
\end{figure}


==> figures/result_real.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width=0.98\linewidth]{images/star_result_real_sensorless.pdf}
	\caption{Comparison between results obtained using networks and baseline on real data.}
	\label{fig:result_real}
\end{figure}


==> figures/result_synthetic.tex <==
\begin{figure*}[tb]
    \centering
    \includegraphics[width=0.93\linewidth]{images/star_result_baseline_2.pdf}
	\caption{Comparison between results obtained using networks and baseline.}
	\label{fig:result_synthetic}
\end{figure*}


==> figures/star_result_l.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width=0.95\linewidth]{images/star_l_curve_16n.pdf}
	\caption{Comparison between results obtained using networks trained with different representations of cluster information.}
	\label{fig:star_result_l}
\end{figure}

